Sketched Adaptive Federated Deep Learning: A Sharp Convergence Analysis

Combining gradient compression methods (e.g., CountSketch, quantization) and adaptive optimizers (e.g., Adam, AMSGrad) is a desirable goal in federated learning (FL), with potential benefits on both fewer communication rounds and less per-round communication. In spite of the preliminary empirical success of sketched adaptive methods, existing convergence analyses show the communication cost to have a linear dependence on the ambient dimension, i.e., number of parameters, which is prohibitively high for modern deep learning models. In this work, we introduce specific sketched adaptive federated learning (SAFL) algorithms and, as our main contribution, provide theoretical convergence analyses in different FL settings with guarantees on communication cost depending only logarithmically (instead of linearly) on the ambient dimension. Unlike existing analyses, we show that the entry-wise sketching noise existent in the preconditioners and the first moments of SAFL can be implicitly addressed by leveraging the recently-popularized anisotropic curvatures in deep learning losses, e.g., fast decaying loss Hessian eigen-values. In the i.i.d. client setting of FL, we show that SAFL achieves asymptotic $O(1/\sqrt{T})$ convergence, and converges faster in the initial epochs. In the non-i.i.d. client setting, where non-adaptive methods lack convergence guarantees, we show that SACFL (SAFL with clipping) algorithms can provably converge in spite of the additional heavy-tailed noise. Our theoretical claims are supported by empirical studies on vision and language tasks, and in both fine-tuning and training-from-scratch regimes. Surprisingly, as a by-product of our analysis, the proposed SAFL methods are competitive with the state-of-the-art communication-efficient federated learning algorithms based on error feedback.

==> arxiv/sections/heavy_tail_noise.tex <==
\vspace*{-2mm}
In this section, we study the performance of Sketched Adaptive Clipped FL (SACFL) defined in Algorithm~\ref{alg:clip} in the context of heavy-tailed noise over gradient norms. This is arguably the more challenging setting and requires carefully addressing the noises with clipping. % need suitable modifications to the proposed SAFL alorithm discussed in Section~\ref{sec:mild}.

\vspace*{-2mm}
\subsection{Heavy-tailed Noise and Sketched Clipping-based Adaptive Methods}
 We start with the key bounded $\alpha$-moment assumption for the heavy-tailed stochastic first-order oracle.
 \vspace*{-3mm}
\begin{assumption}
(Bounded $\alpha$-Moment). There exists a real number $\alpha \in (1,2]$ and a constant $G \ge 0$, such that $\e [\norm{\nabla \cL^c(x, \xi)}^\alpha] \le G^\alpha $, $\forall c \in [C], x \in \mathbb{R}^d$, where $\xi$ is the noise from the  minibatch. 
\label{assume_heavy_tail}
\vspace*{-2mm}
\end{assumption}

Assumption~\ref{assume_heavy_tail} implies that the noise can have unbounded second moments when $\alpha < 2$, which is much weaker compared to Assumption~\ref{a:bcg}. This assumption can be satisfied by a family of noises  including the Pareto 
distribution~\citep{arnold2014pareto} and $\alpha$-stable Levy distribution~\citep{nolan2012stable}, both of which have unbounded variances. Heavy-tailed noises have detrimental effects on most of existing optimization theories, while, at the same time, being prevalent in FL due to data heterogeneity, i.e., non-i.i.d.~client data distributions. This phenomenon has been shown in~\citep{charles2021large}, and Assumption~\ref{assume_heavy_tail} has been adopted in existing theoretical analysis~\citep{zhang2020adaptive,yang2022taming}. %In this regard, adaptive methods have unique advantages in dealing with such heavy-tailed noises. 
Clipping-based methods~\citep{koloskova2023revisiting}, a mainstream approach to handle exceedingly large gradient norms, use adaptive learning rates to normalize the gradient. These methods have empirically demonstrated the capability under heavy-tailed scenarios and are also proven to have optimal convergence rates~\citep{zhang2020adaptive, liu2022communication}.

%clipping based adaptive methods~\cite{} are shown to be effective in dealing with heavy-tail noises. The intuition is that 

\begin{algorithm}[t]
  \SetAlgoLined
  \KwData{Learning rate $\lr$, $\eta$, initial parameters $x_0$, clipping threshold $\tau$.}
  \KwResult{Updated parameters $x_T$}
  Initialize client initial parameters: $x_{0,0}^c = x_0$, $\forall c \in [C]$; \;\\
  \For{$t = 1, 2, \ldots, T$}{
    {\bf Client Updates:}\\
    \For {$c=1,2,\ldots, C$}{
        De-sketch the updates:
        $x_{t,0}^c = x_{t-1} - \lr \min\{\frac{\tau}{\barv_t} , 1\}\decomp( \barm_t)$;
        
        \For {$k=1,2,\ldots,K$}{
        Compute stochastic gradient $g_{t,k-1}^c$ with respect to the parameters $x_{t,k-1}^c$;\\
        Perform a single gradient step:
        $
        x_{t,k}^c = x_{t,k-1}^c - \eta g_{t,k}^c$;
        }
        Sketch the parameter updates:
        \[
        \barm_{t}^c = \comp (x_{t,0}^c - x_{t,K}^c); ~~~~~~\barv_{t}^c = \Vert x_{t,K}^c - x_{t,0}^c\Vert;
        \]
    }
    {\bf Server Updates:}\\Average client updates and send back the averages:%\abcomment{mention this is the server update ... use comments}
    \[
    \barm_t = \frac{1}{C}\sum_{c=1}^C \barm_{t}^c; ~~~~~~\barv_t = \frac{1}{C}\sum_{c=1}^C \barv_{t}^c;
    \]
    Update paramters and statistics:
    $
    x_{t} = x_{t-1} - \lr \min\{\frac{\tau}{\barv_t} , 1\}\decomp( \barm_t).
    $
  }
  \caption{Sketched Adaptive Clipped Federated Learning (SACFL)}
  \label{alg:clip}
\end{algorithm}



Our goal is to apply the sketching techniques to the clipping-based adaptive methods. This is indeed a challenging task. As we have already shown in Section~\ref{sec:mild}, random sketching introduces a significant amount of noise to the client updates. It is unknown whether these noises additionally introduced by sketching will affect the behavior of clipping methods, given that the intrinsic noises are already heavy-tailed due to data heterogeneity.

To address this open question, we propose the Sketched Adaptive Clipped Federated Learning (SACFL) in Algorithm~\ref{alg:clip}. In each round, besides sketching the local updates, the client directly sends the $L_2$-norm of the update to the server. The $L_2$-norm can be viewed as a global second moment specific to clipping methods. Notably, the $L_2$-norm is a scalar value and does not require any compression. Upon receiving the running moments $\barm_t^c, \barv_t^c$ from clients, the server averages the sketched local updates and the $L_2$-norms respectively, and then updates the global model by $x_{t} = x_{t-1} - \lr \min\{\frac{\tau}{\barv_t} , 1\}\decomp( \barm_t)$, where $\lr$ is the learning rate and $\tau$ is a horizon-dependent clipping threshold. When the averaged gradient norm exceeds $\tau$, i.e., when the gradient is in the heavy-tailed regime, clipping is enabled to downscale the gradient. Otherwise, the recovered gradients are directly used to update the global model.
%differs from the standard SGD training algorithms by an additional adaptive clipping operator, which essentially scales the learning rate adaptively. Specifically, the learning rate is set to be two-sided. When the averaged gradient norm exceeds a horizon-dependent threshold $\tau$, i.e., when the gradient is in the heavy-tail regime, clipping is enabled to downscale the gradient. Otherwise, the recovered gradients are directly used to update the global model.


% Note that the clipping operator keeps the relative scales of the gradient norms across clients, while simultaneously normalizing the local updates.

%The clients can be agnostic to the data heterogeneity, and run the optimizers without modifying the gradient.

%\vspace*{-2.5mm}
\subsection{Convergence Analysis}
Next, we state the convergence guarantees of SACFL under Assumption~\ref{assume_heavy_tail}. All technical proofs for this section are in Appendix~\ref{app:heavy}. We start with the descent lemma for clipping methods. 
\begin{lemma}
    If the sketching dimension $b$ satisfies $b \ge 4\log^3(d/\delta)$, taking expectation over the stochasticity of gradients yields, with probability $1-\Theta(\delta)$,
    \begin{align*}
        &\E[\cL(x_{t+1})] - \cL(x_t) +  \frac{\lr \eta K}{4}\norm{\nabla \cL(x_t)}^2 \\ 
        &\le   \frac{\lr \eta K}{2} \norm{\nabla \cL(x_t) - \frac{1}{K} \sumv{C} \E[\tdelta]}^2 
        + \frac{\lr^2 \eta^2}{2} \E[(\frac{1}{C} R^\top R \sum_{c=1}^C \tilde{\Delta}_{t}^c)^\top H_\cL(\hat{x}_t) (\frac{1}{C} R^\top R \sum_{c=1}^C \tilde{\Delta}_{t}^c)], % ~~w.p.~ 
    \end{align*}
    \label{descent_heavy_tail}
    where $\tilde{\Delta}_{t}^c = \min\{1, \frac{\tau}{\sumv{C}\Vert\Delta_t^c\Vert}\}\Delta_t^c$, and $\Delta_t^c = \sum_{k=1}^K g_{t,k}^c$, $ H_{\cL}(\hat{x}_t)$ is the loss Hessian at some $\hat{x}_t$ within the element-wise interval of $[x_t, x_{t+1}]$. %is defined in Appendix~\ref{app_heavy}.
%\vspace*{-2mm}
\end{lemma}
%\abcomment{what is the loss Hessian $\hat{H}_L$ on?}

Intuitively, the first-order terms are barely affected by the heavy-tailed noise since we assume $\alpha > 1$ and these terms do not involve the potentially-unbounded second moments, although special attention for the first-order terms is necessary to achieve the optimal convergence rate, which are deferred to the appendix. Next, we show how to deal with the second-order term. With probability $1-\Theta(\delta)$,
\begin{small}
\begin{align*}
    &\E[(\frac{1}{C} R^\top R \sum_{i=1}^C \tilde{\Delta}_{t}^c)^\top \hat{H}_\cL (\frac{1}{C} R^\top R \sum_{i=1}^C \tilde{\Delta}_{t}^c)] = \E[\sum_{j=1}^d \lambda_j \langle \frac{1}{C} R^\top R \sum_{i=1}^C \tilde{\Delta}_{t}^c , v_j\rangle^2] \\
    %&\le \E[\sum_{j=1}^d  \lambda_j 1_{\lambda_j  \ge 0} \langle \frac{1}{C} R^\top R \sum_{i=1}^C \tilde{\Delta}_{t}^c , v_j\rangle^{2-\alpha} \langle \frac{1}{C} R^\top R \sum_{i=1}^C \tilde{\Delta}_{t}^c , v_j\rangle^{\alpha}] \\
    &\le \E\left[\sum_{j=1}^d  \lambda_j 1_{\lambda_j  \ge 0} \left(\frac{\tau M}{\sumv{C} \norm{\odelta} } \sumv{C} \norm{\odelta} \right)^{2-\alpha} \left(\frac{M}{C} \sum_{i=1}^C \norm{\odelta}\right)^{\alpha}\right] 
     \le M\sum_{j=1}^d  \lambda_j 1_{\lambda_j  \ge 0} K^2 \tau^{2-\alpha}G^\alpha,
\end{align*}
\end{small}
where $M := (1+\logd)$. The first equality follows by using the same eigen-decomposition as in the previous section where $\{\lambda_j,  v_j\}$ are the eigenpairs of $H_\cL(\hat{x}_t)$ and the second order term can be reduced to a squared inner product term. The primary trick thereafter (in the first inequality) is to split the inner product terms into two parts, which can be handled by the two-sided adaptive learning rates respectively. By resorting to the bounded second moment of random sketching, we find the first part with order $2-\alpha$ is contained in a $(1+\logd)\tau-$ball with high probability, and the second part with order $\alpha$ is bounded by applying Assumption~\ref{assume_heavy_tail}. %by putting the two parts together.

\begin{remark}
\normalfont
The bound is high-probability w.r.t the randomness of sketching functions, while the expectation is over other randomness, including local stochastic noises and the heavy-tailed noises. 
\end{remark}

Finally, we can derive the convergence rate for SACFL by combining the analysis. 
\begin{theorem}
    If the sketch size $b$ satisfies $b \ge 4\log^3(dT/\delta)$, then under Assumption \ref{assume_hessian} and \ref{assume_heavy_tail}, the sequence $\{x_t\}$ generated by Algorithm~\ref{alg:clip} (SACFL) satisfies:
    \begin{align*}
        \frac{1}{T}\sum_{t=1}^T \E[\norm{\nabla \cL(x_t)]}^2 \le \frac{4 (\cL(x_1) - \cL(x_T))}{\kappa \eta KT} &+ 3K^2(L^2 \eta^2 G^2 + G^{2\alpha} \tau^{-2(\alpha-1)} + L\eta G^{1+\alpha} \tau^{1-\alpha}) \\
        &+ 3 \sumL \lr \eta(K G^\alpha \tau^{2-\alpha}), ~~w.p.~ 1-\Theta(\delta)
    \end{align*}
    With a proper choice of hyper-parameters with $\lr = K^{\frac{3\alpha-6}{3\alpha-2}}T^{-\frac{1}{3\alpha-2}}$, $\eta= T^{\frac{1-\alpha}{3\alpha-2}}K^{\frac{4-4\alpha}{3\alpha-2}}$ and $\tau=(K^4T)^{\frac{1}{3\alpha-2}}$, we achieve $\frac{1}{T}\sum_{t=1}^T\E[\norm{\nabla \cL(x_t)}^2] \le O(T^{\frac{2-2\alpha}{3\alpha-2}} K^{\frac{4-2\alpha}{3\alpha-2}}),~~w.p.~ 1-\Theta(\delta).$
    \label{theorem_heavy_tail}
\end{theorem}

\begin{remark}
\normalfont
   The convergence rate depends on the noise level $\alpha$. When $\alpha=2$, i.e. the bounded variance case, the convergence rate is $O(1/\sqrt{T})$, which matches the rate in Theorem~\ref{theorem_mild}.  We also claim that the iteration complexity matches the optimal bound in the heavy-tailed case~\citep{yang2022taming, zhang2020adaptive}.  \qed 
\end{remark}


==> arxiv/sections/mild_noise_obsolete.tex <==
In this section, we consider federated learning on nearly-i.i.d client data distribution. The objective is to develop communication-efficient adaptive learning algorithms. We will first propose the general framework for applying gradient compression to \texttt{FedOPT}, and proceed with the mild-noise assumptions and convergence analysis of the algorithm.

\subsection{Sketched Adaptive FL}
Algorithm~\ref{alg:sketch_federated} presents a generic framework of communication-efficient adaptive methods. It calls Algorithm~\ref{alg:ams} as a subroutine, which is a single update step of existing adaptive optimizers. We adopt the well-known \texttt{FedOPT} algorithm ~\cite{reddi2020adaptive} with careful modification in its communication steps to ensure lower communication costs and suitability for adaptive methods. Variants of Algorithm~\ref{alg:ams}, like Adam, can be found in Alg.~\ref{alg:adam} in Appendix.



\begin{algorithm}[t]
  \SetAlgoLined
  \KwData{Learning rate $\eta$, Initial parameters $x_0$, Server Optimizer \texttt{SERVER\_OPT}}
  \KwResult{Updated parameters $x_T$}
  Initialize $m_0 = 0$, $v_0 = 0$, $\hat{v}_0 = 0$\;\\
  \For{$t = 1, 2, \ldots, T$}{
    \For {$c=1,2,\ldots, C$}{
        Client model synchronization: %\abcomment{where is ${\rm AMS\_Step}$ defined}
        \[
        x_{t,0}^c, m_{t}^c, v_{t}^c = \texttt{SERVER\_OPT}(x_{t-1,0}^c, m_{t-1}^c, v_{t-1}^c,  \barm_t, \barv_t)
        \]
        \For {$k=1,2,\ldots,K$}{
        Compute stochastic gradient $g_{t,k-1}^c$ with respect to the parameters $x_{t,k-1}^c$;\\
        Perform a single gradient step:
        $x_{t,k}^c = x_{t,k-1}^c - \eta g_{t,k-1}^c$;
        }
        Compress the parameter updates:
        \[
        \barm_{t}^c = \comp (x_{t,0}^c - x_{t,K}^c); ~~~~~~\barv_{t}^c = [\comp(x_{t,K}^c - x_{t,0}^c)]^2
        \]
    }
    Server: Average client updates and send back the averages:   
%    \abcomment{$C$ and $\comp$ can be confusing, if possible use $\text{sk}$ and $\text{desk}$ for the sketch and desketch operations}
    \[
    \barm_t = \frac{1}{C}\sum_{c=1}^C \barm_{t}^c; ~~~~~~\barv_t = \frac{1}{C}\sum_{c=1}^C \barv_{t}^c;
    \]
    Update paramters and statistics: $x_{t}, m_{t}, v_{t} = \texttt{SERVER\_OPT}(x_{t-1}, m_{t-1}, v_{t-1}, \barm_t, \barv_t)$.
  }
  \caption{Sketched Federated Optimizer}
  \label{alg:sketch_federated}
\end{algorithm}

At each round, after $K$ local training steps, client $c$ sends to the server independent copies of the compressed local model updates and the second moments using a  randomized compression operator $\comp$. Notice that both compressed updates reside in the subspace $\mathbb{R}^b$. If $b$ is much smaller than the ambient dimension $d$, i.e. $b \ll d$ without deteriorating the updates too much, the communication cost per round can be reduced from $O(d)$ to $O(b)$. The server retrieves lossy replicates of the updates by projecting the averaged compressed gradients and the second moments back to the ambient dimension $\mathbb{R}^d$. The gradient compression steps differ Algorithm~\ref{alg:sketch_federated} from the subspace training methods~\cite{gressmann2020improving, wortsman2021learning} since we are utilizing the global gradient vector in each round rather than solely optimizing over the manifold predefined by a limited pool of parameters. Depending on the choice of server-side optimizers, the server use the lossy replicates in $\mathbb{R}^d$ and update the running moments (i.e. the momentum and the second moments).% with the average over clients. 
 Meanwhile, the server sends back the averaged moments in $\mathbb{R}^b$ back to the clients so that each client can perform an exactly identical update to its local model. 

%For simplicity, we ignore several cases e.g. partial participation, asynchronous client updates, but the algorithm can be naively extended to adapt to those settings.

%Specifically, the first-order statistics including the gradient and the momentum are updated

%Momentum SGD , Adam-type algorithms
%The framework is designed to ensure lower transmission cost and fitness for adaptive methods, which we describe in the following.

%\abcomment{remarks, especially long remarks, should not be italicised -- change in the preamble}
\begin{comment}
    \begin{remark}
(Model Synchronization).
\normalfont A critical step in federated learning is to synchronize the server and clients.% at the beginning of each round. %Following the seminal work of Local SGD~\cite{stich2018local}, each client independently executes $K$ local iterations before server averaging. This mechanism relies on strict synchronization and is reportedly communication-efficient by permitting flexible transmission frequencies. 
In Algorithm~\ref{alg:sketch_federated}, with the cost of clients maintaining a copy of the running moments, throughout the training process the model parameters are synchronized at the start of each round, i.e. $x_{t,0}^c = x_t, ~\forall c \in [C]$. Since the compressed message can be recovered by the clients using the decompress method in the previous round, the server can return the averaged moments instead of compressing the moments again, which avoids another round of compression error.  \abcomment{the point being made is not very clear}
%If the original gradient is used as in ~\cite{reddi2020adaptive}, there is no need to distinguish between    
\end{remark}
\end{comment}

\begin{comment}
   \begin{remark} (Moment Averaging Mechanism).
\normalfont
    An alternative averaging method in the server update is to keep track of the individual running moments for each client and average the preconditioned gradients, e.g. $\frac{1}{C} \sum_{c=1}^C m_{t}^c / (\sqrt{v_{t}^c} + \epsilon)$ in \texttt{AMSGrad}, as similarly done by ~\cite{chen2023efficient} in the context of quantization. The nonlinearity of adaptive methods makes this option less attractive. If the client model updates were independently scaled by different second moments, it would incur a bias in the model update. Moreover, it would also increase the transmission cost up to $O(C^2)$, as compared to $O(C)$ in Algorithm~\ref{alg:sketch_federated},  for synchronizing each individual preconditioned gradient.
\end{remark} 
\end{comment}


\begin{remark} (Compression Randomness).
\normalfont
In a single round, the compression operators $\comp$ used by each client share the randomness, by using the same random seed. The random seed can be designated by the server at the beginning of each round. The shared randomness is essential for projecting the local model updates to a shared low dimensional subspace, over which direct averaging makes sense. On the other hand, $\comp$ are independent over different rounds to ensure using distinct subspaces.
\end{remark}

\begin{algorithm}[t]
  \caption{\texttt{SERVER\_OPT} (AMSGrad)}
  \SetAlgoLined
  \KwData{Learning rate $\lr$, $\beta_1$, $\beta_2$, Small constant $\epsilon$, iterate $x_t$, sketched moments $\bar{m}_t$, $\bar{v}_t$}\\
  \KwResult{Updated parameters $\x_{t+1}$}
  Initialize $m_0 = 0$, $v_0 = 0$, $\hat{v}_0 = 0$;\;
  
    Update first moment estimate:~~ $m_t = \beta_1 \cdot m_{t-1} + (1 - \beta_1) \cdot \decomp(\bar{m}_t)$;
    
    Update second moment estimate:~~ $v_t = \beta_2 \cdot v_{t-1} + (1 - \beta_2) \cdot \decomp(\bar{v}_t)$;
    
    Update maximum of past second moment estimates: 
    $\hat{v}_t = \max(\hat{v}_{t-1}, v_t).$
    
    Update parameters:
    $x_{t+1} = x_{t} - \frac{\lr}{\sqrt{\hat{v}_t} + \epsilon} \cdot m_t := x_t - \kappa {\hat{V}_{t}}^{-1/2} m_t$.
  %}
  \label{alg:ams}
%\vspace*{-3mm}
\end{algorithm}

\begin{comment}
    \begin{algorithm}[t]
  \caption{AMS\_Step}
  \SetAlgoLined
  \KwData{Learning rate $\lr$, $\beta_1$, $\beta_2$, Small constant $\epsilon$, iterate $x_t$}
  \KwResult{Updated parameters $\x_{t+1}$}
  Initialize $m_0 = 0$, $v_0 = 0$, $\hat{v}_0 = 0$\;
  %\For{$t = 1, 2, \ldots, T$}{
    %Compute gradient $g_t$ with respect to the parameters $x_{t-1}$\;
    Update first moment estimate:
    \[
    m_t = \beta_1 \cdot m_{t-1} + (1 - \beta_1) \cdot \decomp(\bar{m}_t)
    \]
    Update second moment estimate:
    \[
    v_t = \beta_2 \cdot v_{t-1} + (1 - \beta_2) \cdot \decomp(\bar{v}_t)
    \]
    Update maximum of past second moment estimates: 
    \[
    \hat{v}_t = \max(\hat{v}_{t-1}, v_t)
    \]
    Update parameters:
    \[
    x_{t+1} = x_{t} - \frac{\lr}{\sqrt{\hat{v}_t} + \epsilon} \cdot m_t := x_t - \kappa {\hat{V}_{t}}^{-1/2} m_t
    \]
  %}
  \label{alg:ams}
\end{algorithm}
\end{comment}


\subsection{Random Sketching}
So far, we haven't discussed any specific compression techniques used in each round of communication. We will first introduce the desired characteristics of compression and then list a family of sketching algorithms which possess those properties.

\begin{property} (Linearity). The compression operators are linear with regard to the input vectors, i.e. $\comp(\sum_{i=1}^n {v_i}) = \sum_{i=1}^n {\comp(v_i)}$  and   $\decomp(\sum_{i=1}^n {\bar{v}_i}) = \sum_{i=1}^n {\decomp(\bar{v}_i)},~~ \forall \{v_i\}_{i=1}^n, \{\bar{v}_i\}_{i=1}^n$.
\end{property}

\begin{property} (Unbiased Estimation).
    For any vector $v \in \mathbb{R}^d$, $\E[\decomp(\comp(v))] = v$.
\end{property}

\begin{property} (Bounded Vector Products).
\label{property_vector_product}
    For any fixed vector $v, h \in \mathbb{R}^d$, $\P(\vert \langle \decomp(\comp(v)), h \rangle - \langle v, h \rangle \vert \ge (\logd)\norm{v}\norm{h}) \le \Theta(\delta)$.
\end{property}
%\abcomment{this is not a second moment bound, the variance will depend on the ambient dimension}

Property 1 and 2 guarantee the average of moments in Algorithm~\ref{alg:sketch_federated} over clients are, in expectation, the same as those in \texttt{FedOPT}. Property 3 quantifies the bound on the deviation of applying compression to vector products. We find that letting $\comp(v) = Rv$ and $\decomp(v) = R^\top v$, where $R \in \R^{b \times d}$ is the random sketching operators, can satisfy all the properties above. Different instantiations of $R$ generate a rich family of sketching operators, including Gaussian, SRHT~\cite{lu2013faster}, Count-Sketch~\cite{charikar2002finding} etc. 

%The algorithm can be reduced to the original adaptive federated optimization~\cite{reddi2020adaptive} if the sketching and de-sketching algorithm are identity mappings.

%\begin{remark} (Sketching Second Moment). \normalfont In Algorithm~\ref{alg:sketch_federated}, sketching of the  second moment is operated over the squared gradient, i.e $R^\top R g^2$. Another plausible approach is to directly take square of the recovered gradient, i.e. $(R^\top Rg)^2$. It can be proven that %\abcomment{can be proved for random sketches}, 
%random sketching methods achieve $O(d)$ bounds on $\vert \langle \decomp(\comp(v))^2, h \rangle - \langle v^2, h \rangle \vert$, while using $R^\top R g^2$ introduces merely a $\log(d)$ factor. 
% Notice that there is no guarantee that  $RRg^2$ will be positive in all elements, although its expectation is non-negative. That's why we need a $\max$ operator.
    
%\end{remark}

\subsection{Convergence Analysis}
Before conducting the convergence analysis for Algorithm~\ref{alg:sketch_federated}, we first state several standard assumptions that are commonly used in the literature of first-order stochastic methods. Specifically, we first focus on mild noise, which is typically observed when the training data are nearly i.i.d across clients.

\begin{assumption} (Bounded Global Gradients). Square norm of the gradient is uniformly bounded, i.e. $\Vert \nabla \cL(x) \Vert^2 \le G_g^2$.
\label{a:bgg}
\end{assumption}

%This is a standard assumption widely used in various distributed learning literatures~\cite{reddi2020adaptive} and adaptive gradient methods ~\cite{}.

\begin{assumption} (Bounded Client Gradients).
For every client, there exists a constant $G_c \ge 0$,  such that $\Vert \nabla \cL^c(x) \Vert^2 \le G_c^2, ~c \in [C]$.
\label{a:bcg}
\end{assumption}
\begin{comment}
    \begin{remark}
\normalfont
    %We call the variance induced by data heterogeneity satisfying Assumption \ref{a:bcg} as mild noise.
    Assumption \ref{a:bcg} depicts the level of noise induced by data heterogeneity. Together with Assumption \ref{a:bgg}, Assumption \ref{a:bcg} can be transformed to the bounded variance condition commonly used in federated optimization, i.e. $\sumv{C}\norm{\nabla \cL^c(x) - \nabla \cL(x)}^2 \le \frac{2}{C}\sum_{c=1}^C(\norm{\nabla \cL^c(x)}^2 + \norm{\nabla \cL(x)}^2) \le 2G +  \frac{2}{C}\sum_{c=1}^C G_c^2$. The bounded client gradient assumption can characterize data \abcomment{limited?} heterogeneity across clients. In i.i.d. settings where the data of each client have the same distribution, i.e. $\norm{\nabla \cL^c(x) - \nabla \cL(x)}^2 = 0$, we have $G_g = G_c, ~\forall c \in [C]$.\abcomment{not sure I follow: is $\cL$ the population loss or finite sample loss? what about $\cL^c$?} %[We are avoiding expectation in this section. $\cL$ is just the loss over all the samples, and $\cL^c$ is the loss over the client dataset.]
    %Hence, the bounded client gradient represents data heterogeneity across clients. In i.i.d settings where the data of each client have the same distribution, $\e [\norm{\nabla \cL_i(x) - \nabla \cL(x)}^2] = 0$, which implies $G_i = G$.
\end{remark}
\end{comment}


For simplicity, we use a unified notation $G := \max \{ \max\{G_c\}_{c=1}^C, G_g\}$ to denote the upper bound for client and global gradient norms. We also assume the stochastic noise in min-batch settings is sub-Gaussian, which is widely used in various first-order optimization~\cite{harvey2019tight,mou2020linear}.

\begin{assumption} (Sub-Gaussian Noise).
The stochastic noise $\norm{\nabla \cL^c(x) - g^c(x)}$ at each client is a $\sigma-$sub-Gaussian random variable, i.e. $\P(\norm{\nabla \cL^c(x) - g^c(x)} \ge t) \le 2 \exp(-t^2/\sigma^2)$, for all $t\ge 0$.
\label{assume_local_grad_sub}
\end{assumption}

Besides, we have assumptions on the Hessian eigenspectrum $\{\lambda_i, v_i\}_{i=1}^d$ of the loss function $\cL$.
\begin{assumption} (Hessian Matrix Eigenspectrum)
    The smoothness of the loss function $\cL$, i.e. the largest eigenvalue of the loss Hessian $H_\cL$ is bounded by $L$, $\max_i \lambda_i \le L$. The sum of absolute values of  $H_\cL$ eigenspectrum is bounded by $\sumL$, i.e. $\sum_{i=1}^d \vert \lambda_i \vert \le \hat L$.
    \label{assume_hessian}
\end{assumption}

Assumption~\ref{assume_hessian} on smoothness directly leads to $\Vert \nabla \cL(x_1) - \nabla\cL(x_2)\Vert \le L\norm{x_1 - x_2}$\abcomment{for deep learning models, we use $\theta$ for the parameters and $x$ for the input -- may be hard to change things now}. The assumption of bounded sum of eigenspectrum has been validated by several recent literatures~\cite{xie2022power, li2020hessian}, where the eigenspectrum is observed to conform with a power-law distribution. An empirical verification under the setting of FL can be found in Fig.~\ref{fig:vit-small-eigenspectrum} in the Appendix.

Now we can derive the convergence analysis of Algorithm~\ref{alg:sketch_federated} as in Theorem~\ref{theorem_mild}.
\begin{theorem}
    Suppose the sequence of iterates $\{x_t\}_{t=1}^T$ is generated by Algorithm~\ref{alg:sketch_federated}. Under Assumptions 1-4, with probability $1 - \Theta(\delta) - O(\exp(-\Omega(\lambda^2))) -\delta_g $,\abcomment{what is $\lambda, \delta_g$?}
    \begin{small}
    \begin{align*}
    &\left(\sqrt{1+\logtdsq} \eta K G + \epsilon \right)^{-1} \lr \eta KT \Vert \nabla \cL (x_t) \Vert^2  
    \leq \cL(z_1) + \frac{1}{\epsilon} \lr \eta^2 L K^2G^2 T \\ &+ \lambda \lr \eta K\sqrt{T}(\logtd \frac{G^2}{\epsilon} + \frac{1}{\epsilon\sigma}\log(\frac{2T}{\delta_g})) 
    + \eta^2 \kappa^2 T (1+\logtd)^2 \frac{8}{(1-\beta_1)^2} \frac{\sumL K^2 G^2}{\epsilon^2},
    \end{align*}   
    \end{small}
    where $\delta, \lambda$, and $\delta_g$ are the randomness from sketching, sub-Gaussian stochastic noise and martingales respectively.
    % \begin{align*}
    % &\left(\sqrt{1+\logtdsq} \eta K G + \epsilon \right)^{-1} \lr \eta KT \Vert \nabla \cL (x_t) \Vert^2  \\
    % \le& \cL(z_1) + \frac{1}{\epsilon} \lr \eta^2 L K^2G^2 T + \lambda \lr \eta K\sqrt{T}(\logtd \frac{G^2}{\epsilon} + \frac{1}{\epsilon\sigma}\log(\frac{2T}{\delta_g})) 
    % \\
    % &+ \eta^2 \kappa^2 T (1+\logtd)^2 \frac{8}{(1-\beta_1)^2} \frac{\sumL K^2 G^2}{\epsilon^2}.
    % \end{align*}
    \label{theorem_mild}
\end{theorem}
\begin{remark}
\normalfont
    By Theorem~\ref{theorem_mild}, we can achieve an asymptotic $O(T^{-1/2})$ iteration complexity by setting $\eta = O(T^{-1/2}K^{-1})$ and $\kappa=O(1)$.
\end{remark}


\subsection{Technical Overview}
The proof of Theorem~\ref{theorem_mild} contains several critical components, which are unique to adaptive methods. We follow the common proof framework of adaptive optimization, and carefully deal with the noise introduced by random sketching in both momentum and second moments. We adopt AMSGrad~\cite{reddi2019convergence} as the server optimizer and it would be straightforward to extend the analysis to other adaptive methods.

We first introduce the descent lemma for AMSGrad. For conciseness, we denote the precondtioner matrix ${\rm diag}((\sqrt{v_t}+\epsilon)^2)$ as $\hat{V}_t$. Define auxiliary variable $z_t = x_t + \frac{\beta_1}{1-\beta_1}(x_t - x_{t-1})$. The trajectory of $\cL$ over $\{z_t\}_{t=1}^T$ can be tracked by the following lemma.
\begin{lemma}
\label{lemma_descent_amsgrad}
    For any round $t \in [T]$, there exists function $\Phi_t \ge 0$ ,and $\Phi_0 \le G$ such that the iterates generated by Algorithm~\ref{alg:sketch_federated} using AMSGrad optimizer satisfies
    \begin{align*}
    \cL(z_{t+1}) &\le \cL(z_t) + \Phi_t - \Phi_{t+1} - \frac{\kappa\etat}{C}\sum_{c=1}^C  \sum_{k=1}^K\nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}   R_t^\top R_t g_{t,k}^c + \calQ(z_{t+1}-z_t, z_t - x_t), % \label{eq:single_step_taylor}
    \end{align*}
    where $\calQ(u,v)$ is a quadratic form defined over $u, v \in \R^d$.
\end{lemma}
Our objective henceforth is to bound the first-order descent term and the second-order quadratic term on the right hand side respectively.

\textbf{Second-Order Quadratic Term.} Denote $\{\lambda_j, v_j \}_{j=1}^d$ as the eigen-pairs of $\hat H_{\cL}$. A sample component of the quadratic form can be written as
\begin{align*}
     (z_{t+1}-z_t)^\top \hat H_{\cL} (z_{t+1}-z_t) = \sum_{j=1}^d \lambda_j \langle z_{t+1}-z_t, v_j \rangle^2,
\end{align*}
where $\hat H_\cL$ is the second-order Taylor remainder. The term can be viewed as the sum of projection of $z_{t+1}-z_t$ onto the eigen-space of $\hat H_{\cL}$. We bound the inner products by the following lemma.
\begin{lemma} For $t \in [T]$. With probability $1-t\delta$,
    \begin{align*}
     \langle z_{t+1}-z_t, v_j \rangle \le \kappa \eta (1+\frac{\log^{1.5}(CKd/\delta)}{\sqrt{b}})\frac{1+\beta_1}{1-\beta_1} \frac{K G}{\epsilon}.
    \end{align*}
    \label{lemma_inner_product}
\end{lemma}
Bounding the inner-product term is non-trivial since $z_t$ contains momentum information which depends on the randomness of previous iterations. A proof of a generalized version of this statement is deferred to the appendix, where induction methods are used to address the dependence. Combining Lemma~\ref{lemma_inner_product} with Assumption~\ref{assume_hessian} yields a dimension-free bound on the second-order quadratic term.

\begin{remark}
\normalfont
A straightforward application of smoothness to the second-order term yields a quadratic term $\norm{R^\top Rg}^2$, which is linearly proportional to $d$ in scale. We avoid this dimension dependence by combining Property~\ref{property_vector_product} of random sketching and Assumption~\ref{assume_hessian}.%However, we have limited knowledge over this quadratic term.
\end{remark}

\begin{comment}
Observe that the loss Hessian can be split into the sum of Gauss-Newton matrix and predictor Hessian. Take mean square error as an example,
\begin{align}
    H_\cL = \frac{1}{N} \sum_{i=1}^N  l_i^{\prime \prime} \nabla f_i \nabla f_i^T + \sum_{i=1}^d l_i^\prime H_{f_i} = \frac{1}{N} \sum_{i=1}^N  \nabla f_i \nabla f_i^T + \sum_{i=1}^d l_i^\prime H_{f_i}
\end{align}
\end{comment}

%\textbf{Induction on Moments.} Noticing that involves momentum, which depends on the in all previous 

\textbf{First-Order Descent Term}. %We can deal with the components of the first order term separately. 
The first-order term in the descent lemma can be decomposed into three components, which we will handle separately:
\begin{small}
\begin{align*}    \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}   R_t^\top R_t g_{t,k}^c =& \underbrace{\nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2} \nabla \cL^c(x_t)}_{\cD_1}  +   \underbrace{\nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2} (R_t^\top R_t g_{t,k}^c - \nabla \cL^c(x_{t,k}^c))}_{\cD_2} \\
    &+  \underbrace{\nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}(\nabla \cL^c(x_{t,k}^c) - \nabla \cL^c(x_t))}_{\cD_3}.
    \label{eq:fod}
%\vspace*{-2mm}
\end{align*}
\end{small}
First, $\cD_3$ %, involves the difference between local iterates and global iterates which 
can be reduced to a second-order term by smoothness over $\cL$,
\begin{small}
\begin{align*}
    \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}(\nabla \cL^c(x_{t,k}^c) - \nabla \cL^c(x_t))
    %=  \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}\hH_L^c(x_{t,k}^c - x_t)
    =  -\eta \sum_{\tau=1}^k \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}\hH_\cL^c g_{t, \tau}^c.
\vspace*{-2mm}
\end{align*}
\end{small}
%
\begin{comment}
\begin{align*}
    \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}(\nabla \cL^c(x_{t,k}^c) - \nabla \cL^c(x_t))
    =  \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}\hH_L^c(x_{t,k}^c - x_t)
    =  -\eta \sum_{\tau=1}^k \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}\hH_\cL^c g_{t, \tau}^c.
\end{align*}

\begin{align*}
    \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2}(\nabla \cL^c(x_{t,k}^c) - \nabla \cL^c(x_t))
    \le \frac{1}{\epsilon}\eta KG^2
\end{align*}
\end{comment}
Note that this term does not involve any stochasticity with regard to random sketching, which means we can directly derive the upper bound by Cauchy-Schwartz. Next, observing that $\sumv{C} \nabla \cL^c(x_t) = \nabla \cL(x_t)$, $\cD_1$ composes a scaled squared gradient norm. Applying element-wise high probability bound on random sketching yields the lower bound for the scale.
\begin{comment}
    \begin{lemma}
    High probability bound on $V_t$
\end{lemma}
Then with high probability,
\end{comment}
\begin{lemma} For ${\hat{V}_{t-1}}^{-1/2}$ generated by Algorithm~\ref{alg:sketch_federated}, with probability $1-\delta$,
\begin{align*}
\nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2} \nabla \cL(x_t) \ge \left(\sqrt{1+\logdsqt} \eta K G + \epsilon \right)^{-1} \Vert \nabla \cL (x_t) \Vert^2.
\vspace*{-2mm}
\end{align*}
\label{lemma_descent_bound}
\end{lemma}
%
% \begin{comment}
%     \begin{align*}
% \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2} \nabla \cL(x_t) %&= \sum_{i=1}^d (\sqrt{\hat{v}_{t,i}} + \epsilon)^{-1}[\nabla \cL(x_t)]_i^2 \\
% & \ge (\sqrt{\max_i [\hat{v}_{t,i}]} + \epsilon)^{-1} \sum_{i=1}^d  [\nabla \cL(x_t)]_i^2 \ge (\logd \eta K G + \epsilon)^{-1} \Vert \nabla \cL (x_t) \Vert^2
% \end{align*}
% \end{comment}
%
\textbf{Martingale for zero-centered noise.} $\cD_2$ contains a zero-centered noise term $R_t^\top R_t g_{t,k}^c - \nabla \cL^c(x_{t,k}^c)$, where the randomness is over $R_t$ and the mini-batch noise at round $t$. Though $x_{t,k}^c$ has temporal dependence, the fresh noise at round $t$ is independent of the randomness in the previous iterations. Hence, the random process defined by the aggregation of these norm terms over time forms a martingale. The martingale difference can be bounded with high probability under our proposed sketching method. Then by adapting Azuma's inequality on a weaker bounding condition, we have :
\begin{lemma}
\label{lemma_martingale}
    With probability $1- O(\exp(-\Omega(\lambda^2))) -\delta -\delta_g$,
\begin{align*}
    \sum_{t=1}^T  \left\vert \frac{1}{C}\sum_{c=1}^C  \sum_{k=1}^K \nabla \cL(x_t)^\top {\hat{V}_{t-1}}^{-1/2} (R_t^\top R_t g_{t,k}^c - \nabla \cL^c(x_{t,k}^c)) \right\vert \le \lambda \sqrt{T}(\logtd \frac{KG^2}{\epsilon} + \frac{1}{\epsilon\sigma}\log(\frac{2T}{\delta_g})).
\end{align*}
\end{lemma}
\begin{comment}
   $P(\vert Y_T \vert \ge \lambda \sqrt{\sum_{t=1}^T \left( \frac{\log^{1.5}(d/\delta)}{\sqrt{b}} G \Vert \hV  \nabla \cL(x_t)\Vert_2\right)^2} ) = O(\exp(-\Omega(\lambda^2))) + T \delta$ 
\end{comment}
Finally, applying union bounds to these parts and telescoping  the descent lemma lead to Theorem~\ref{theorem_mild}.



